LongDocURL: a Comprehensive Multimodal Long Document Benchmark Integrating Understanding, Reasoning, and Locating

Large vision language models (LVLMs) have improved the document understanding capabilities remarkably, enabling the handling of complex document elements, longer contexts, and a wider range of tasks. However, existing document understanding benchmarks have been limited to handling only a small number of pages and fail to provide a comprehensive analysis of layout elements locating. In this paper, we first define three primary task categories: Long Document Understanding, numerical Reasoning, and cross-element Locating, and then propose a comprehensive benchmark, LongDocURL, integrating above three primary tasks and comprising 20 sub-tasks categorized based on different primary tasks and answer evidences. Furthermore, we develop a semi-automated construction pipeline and collect 2,325 high-quality question-answering pairs, covering more than 33,000 pages of documents, significantly outperforming existing benchmarks. Subsequently, we conduct comprehensive evaluation experiments on both open-source and closed-source models across 26 different configurations, revealing critical performance gaps in this field.

==> table/statis_of_dataset.tex <==
\begin{table}[htbp]
    \centering
    \resizebox{0.5\textwidth}{!}{
    \begin{tabular}{lc}
        \toprule
        \textbf{Statistic} & \textbf{Number} \\
        
        \midrule
        \textbf{Document} \\
            ~- Total & 396 \\
            ~- Type & 8 \\
            ~- Avg. pages & 85.6 \\
          
        \midrule
        \textbf{Question \& Answer} \\
            ~- Total & 2,325 \\
            ~- Avg. question tokens\footnotemark[6] & 35.5 \\
            ~- Max. question tokens & 277 \\
        \textcolor{gray}{Task Type} \\
            ~- Understanding & 1,243 (53.5\%) \\
            ~- Reasoning & 387 (16.6\%)  \\
            ~- \Locating & 695 (29.9\%) \\
        \textcolor{gray}{Entity Type} \\ 
            ~- Pure-text & 994 (42.8\%) \\
            ~- Layout & 779 (33.5\%) \\
            ~- Table & 556 (23.9\%) \\
            ~- Figure & 871 (37.5\%) \\
        \textcolor{gray}{Number of Evidence Pages} \\
            ~- Single-page question & 1,093 (47.0\%) \\
            ~- Multi-page questions & 1,230 (52.9\%)  \\
            ~- Unanswerable questions & 2 (0.1\%) \\
        \textcolor{gray}{Number of Evidence Entities} \\
            ~- Single-entity question & 1,463(62.9\%) \\
            ~- Cross-entity question & 862(37.1\%) \\
        \textcolor{gray}{Answer Format} \\ 
            ~- String   & 941 (40.5\%) \\
            ~- Integer  & 431 (18.5\%) \\
            ~- Float & 185 (8.0\%) \\
            ~- List & 757 (32.5\%) \\
            ~- None & 11 (0.5\%) \\
        \bottomrule
    \end{tabular}
    }
    \caption{Dataset statistics}
    \label{tab:statistics}
    \vspace{-5mm}
\end{table}

\footnotetext[6]{We get the number of question tokens using the Qwen2 tokenizer.}
